Modeling Long-Range Context for Concurrent Dialogue Acts Recognition

In dialogues, an utterance is a chain of consecutive sentences produced by one speaker which ranges from a short sentence to a thousand-word post. When studying dialogues at the utterance level, it is not uncommon that an utterance would serve multiple functions. For instance, "Thank you. It works great." expresses both gratitude and positive feedback in the same utterance. Multiple dialogue acts (DA) for one utterance breeds complex dependencies across dialogue turns. Therefore, DA recognition challenges a model's predictive power over long utterances and complex DA context. We term this problem Concurrent Dialogue Acts (CDA) recognition. Previous work on DA recognition either assumes one DA per utterance or fails to realize the sequential nature of dialogues. In this paper, we present an adapted Convolutional Recurrent Neural Network (CRNN) which models the interactions between utterances of long-range context. Our model significantly outperforms existing work on CDA recognition on a tech forum dataset.

==> 16DAlables_table.tex <==
\begin{table}[t]
\small
\caption{16 most frequent DA combinations that occur in more than 1\% of 10,020 utterances (i.e. frequency larger than 100)}
\resizebox{0.47 \textwidth}{!}{   %resize table
\begin{tabular}{lll|lll}
\toprule
Rk. & DAs & Perc. & Rk. & DAs & Perc. \\
\midrule
1 & OQ & 15.30\% & 9 & GG IR PA & 2.10\% \\
2 & PA & 14.10\% & 10 & FD GG PA & 2.00\% \\
3 & GG PA & 10.00\% & 11 & IR PA & 1.60\% \\
4 & GG PF & 5.10\% & 12 & FD GG & 1.50\% \\
5 & GG & 3.50\% & 13 & FD GG PF & 1.50\% \\
6 & GG OQ & 3.20\% & 14 & FD NF & 1.30\% \\
7 & FD PA & 3.10\% & 15 & RQ & 1.20\% \\
8 & FD & 2.90\% & 16 & FD OQ & 1.10\% \\
\bottomrule
\end{tabular}
}
\label{tab:most_frequent_16_DAs_combinations}
\vspace{-4mm}
\end{table}

==> results_table.tex <==

\begin{table*}[t]
\small \centering 
\caption{\label{tab:LSTM_result} Baseline and DAMIC LSTM results with or without utterance collapsing}
\addtolength{\leftskip} {-1cm}
\addtolength{\rigthtskip} {-1cm}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{}} & \multicolumn{1}{c|}{\multirow{2}{*}{F1}} & \multicolumn{12}{c|}{\textbf{F1 per DA}} \\ \cline{4-15} 
\multicolumn{2}{|l|}{} & \multicolumn{1}{c|}{} & CQ & FD & FQ & GG & IR & JK & NF & O & OQ & PA & PF & RQ \\ \hline
\multirow{2}{*}{Baseline} & -collapsed & 51.85 & 16.54 & 49.93 & 28.50 & 49.06 & 32.56 & 7.14 & 22.55 & 1.81 & \textbf{85.35} & \textbf{72.76} & 35.12 & 19.41 \\ \cline{2-15} 
 & +collapsed & 52.48 & 19.04 & 47.81 & 23.73 & \textbf{51.54} & 27.60 & 6.64 & 25.52 & 1.13 & \textbf{86.88} & \textbf{73.86} & 34.68 & 17.56 \\ \hline
\multirow{2}{*}{DAMIC} & -collapsed & 64.39 & 23.83 & \textbf{55.79} & 27.87 & \textbf{75.88} & 34.50 & 8.06 & 32.31 & 3.10 & \textbf{93.60} & \textbf{85.40} & \textbf{50.07} & 34.42 \\ \cline{2-15} 
 & collapsed & \textbf{65.00} & 21.22 & \textbf{52.13} & 27.76 & \textbf{77.91} & 34.86 & 8.93 & 32.54 & 2.09 & \textbf{93.59} & \textbf{85.73} & \textbf{52.99} & 32.14 \\ \hline
\end{tabular}
\end{table*}


==> stats_by_number_DAs.tex <==
\begin{table}[t]
\small \centering 
\resizebox{0.5 \textwidth}{!}{ 
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\# of \\ DAs\end{tabular}} & \multirow{2}{*}{\%} & \multicolumn{5}{c|}{Number of tokens} \\ \cline{3-7} 
 &  & Mean & Median & SD  & Min & Max \\ \hline
1 & 40.05 & 65.80 & 47 & 71.95 & 1 & 1028 \\ \hline
2 & 40.75 & 69.16 & 51 & 69.63  & 1 & 971 \\ \hline
3 & 15.73 & 87.13 & 65 & 78.16  & 4 & 654 \\ \hline
4 & 3.03 & 103.16 & 76.5 & 87.19 & 7   & 846 \\ \hline
5 & 0.38 & 136.34 & 119 & 85.66  & 21 & 386 \\ \hline
6 & 0.06 & 176.50 & 177 & 93.18  & 47 & 324 \\ 
% \bottomrule[0.4mm]
% macro & 100\% & 71.99 & 53.00 & 73.32 & 1 & 1028 \\
\bottomrule
\end{tabular}
}
\caption{Correlation between number of concurrent DAs and utterance length}
\label{tab:number_DA_combo_freq_utterance_length}

\end{table}
